KMC 2: Fast and resource-frugal $k$-mer counting

Motivation: Building the histogram of occurrences of every $k$-symbol long substring of nucleotide data is a standard step in many bioinformatics applications, known under the name of $k$-mer counting. Its applications include developing de Bruijn graph genome assemblers, fast multiple sequence alignment and repeat detection. The tremendous amounts of NGS data require fast algorithms for $k$-mer counting, preferably using moderate amounts of memory. Results: We present a novel method for $k$-mer counting, on large datasets at least twice faster than the strongest competitors (Jellyfish~2, KMC~1), using about 12\,GB (or less) of RAM memory. Our disk-based method bears some resemblance to MSPKmerCounter, yet replacing the original minimizers with signatures (a carefully selected subset of all minimizers) and using $(k, x)$-mers allows to significantly reduce the I/O, and a highly parallel overall architecture allows to achieve unprecedented processing speeds. For example, KMC~2 allows to count the 28-mers of a human reads collection with 44-fold coverage (106\,GB of compressed size) in about 20 minutes, on a 6-core Intel i7 PC with an SSD. Availability: KMC~2 is freely available at http://sun.aei.polsl.pl/kmc. Contact: sebastian.deorowicz@polsl.pl

==> pseudo.tex <==
\clearpage
\section{Pseudocodes of the KMC algorithm}
\label{sec:pseudo}

% ***** FASTQ reader
\begin{figure}[h]
\begin{algorithm}{\algdef{FASTQ-reader}(\textit{FL\_queue})}
\pcinput{{FL\_queue} --- queue with list of input file names}\\
\pcendparam
\lno \pcwhile (\textit{file\_name} $\gets$ \textit{FL\_Queue}.pop()) \pcnot empty \pcdo\\
\lno\>	\textit{file} $\gets$ Open file \textit{file\_name}\\
\lno\>	\pcwhile (\textit{block} $\gets$ \textit{file}.read\_next\_block()) \pcnot empty \pcdo\\
\lno\>\>		\textit{FASTQ\_parts\_queue}.push(\textit{block})\\
\lno\>	Close \textit{file}
\end{algorithm}
\caption{Reading FASTQ/FASTA files. Each block, of several megabytes, is rounded to the nearest complete read.
The blocks are inserted into a FASTQ parts queue.}
%% \caption{Pseudocode of algorithm reading FASTQ/FASTA files. Block sizes are adjusted at the start of the algorithm
%% according to available memory and typically are in range 4--16\,MB. After reading a block it is adjusted to the last
%% complete read. The remaining part starts the next block}
\label{code:fastq_reader}
\end{figure}


% ***** Splitter
\begin{figure}[h]
\begin{algorithm}{\algdef{Splitter}(\textit{FASTQ\_parts\_queue})}
\pcinput{{FASTQ\_parts\_queue} --- queue with parts of FASTQ/FASTA files}\\
\pcendparam
\lno \pcwhile (\textit{block} $\gets$ \textit{FASTQ\_parts\_queue}.pop()) \pcnot empty \pcand \pcnot \textit{FASTQ\_parts\_queue}.finished() \pcdo\\
\lno\>	\pcif \textit{block} \pcnot empty \pcthen\\
\lno\>\>		\pcforall \textit{read} in \textit{block} \pcdo\\
\lno\>\>\>		\pcforall valid indices $i$ in \textit{read} \pcdo\\
\lno\>\>\>\>		Compute canonical $k$-mer \textit{m} (together with quality-based counter for Quake's mode)\\
\lno\>\>\>\>		\textit{bin\_id} $\gets$ \textit{prefix}($m$, $p_1$)\\
\lno\>\>\>\>		\textit{bin}[\textit{bin\_id}].push($m$ without prefix)\\
\lno\>\>\>\>		\pcif \textit{bin}[\textit{bin\_id}] is full \pcthen\\
\lno\>\>\>\>\>			Compact \textit{bin}[\textit{bin\_id}] by sorting on $p_2$ symbols\\
\lno\>\>\>\>\>			\textit{Bin\_parts\_queue}.push(\textit{bin\_id}, compacted \textit{bin}[\textit{bin\_id}])\\
\lno\>\>\>\>\>			Empty \textit{bin}[\textit{bin\_id}]\\
\lno \pcforall valid indices $i$ in \textit{bin} \pcdo\\
\lno\>			Compact \textit{bin}[\textit{i}] by sorting on $p_2$ symbols\\
\lno\>			\textit{Bin\_parts\_queue}.push(\textit{i}, compacted \textit{bin}[\textit{i}])\\
\lno\>			Empty \textit{bin}[\textit{i}]
\end{algorithm}
\caption{Algorithm of splitting $k$-mers in reads to bins according to their prefix.
A full bin is compacted by sorting on $p_2$-symbol prefix, and removing this prefix.} 
%% \caption{Pseudocode of algorithm splitting $k$-mers in reads to bins according to their prefix.
%% When some bin gets full (bin size is adjusted according to available memory, but typical values are $2^{14}$ or 
%% $2^{15}$ entries) it is compacted by sorting on $p_2$-symbol prefix, and removing this prefix}
\label{code:splitter}
\end{figure}



% ***** Package maker
\begin{figure}[h]
\begin{algorithm}{\algdef{Package-Maker}(\textit{Bin\_parts\_queue})}
\pcinput{{Bin\_parts\_queue} --- queue with parts of FASTQ/FASTA files}\\
\pcendparam
\lno \pcwhile (\textit{bin\_id}, \textit{bin\_part} $\gets$ \textit{Bin\_parts\_queue}.pop()) \pcnot empty \pcand \pcnot \textit{Bin\_parts\_queue}.finished() \pcdo\\
\lno\>	\pcif \textit{bin\_part} \pcnot empty \pcthen\\
\lno\>\>	Put \textit{bin\_part} to \textit{bin\_package}[\textit{bin\_id}]\\
\lno\>\>	\pcif Size of \textit{bin\_package}[\textit{bin\_id}] $>$ maximal size of single package \pcthen\\
\lno\>\>\>		\textit{Bin\_part\_packages\_queue}.push(\textit{bin\_id}, \textit{bin\_package}[\textit{bin\_id}])\\
\lno\>\>	\pcif Total size of all bin packages $>$ maximal amount of memory for package maker \pcthen\\
\lno\>\>\>			$i$ $\gets$ id of largest bin package in \textit{bin\_package} array\\
\lno\>\>\>		\textit{Bin\_part\_packages\_queue}.push($i$, \textit{bin\_package}[\textit{i}])\\
\lno	\pcforall valid indices $i$ in \textit{bin\_package} \pcdo\\
\lno\>		\textit{Bin\_part\_packages\_queue}.push($i$, \textit{bin\_package}[\textit{i}])
\end{algorithm}
\caption{Algorithm of collecting compacted bin parts from all splitting threads.} 
%% \caption{Pseudocode of algorithm collecting compacted bin parts from all splitting threads.}
\label{code:package_maker}
\end{figure}


% ***** Compactor
\begin{figure}[h]
\begin{algorithm}{\algdef{Compactor}(\textit{...})}
\pcinput{{...} --- queue with parts of FASTQ/FASTA files}\\
\pcendparam
\lno \pcwhile (\textit{bin\_id}, \textit{bin\_package} $\gets$ \textit{Bin\_part\_packages\_queue}.pop()) \pcnot empty \pcand\\ 
\>\>\pcnot \textit{Bin\_part\_packages\_queue}.finished() \pcdo\\
\lno\>	\pcif \textit{bin\_package} \pcnot empty \pcthen\\
\lno\>\>		Try to compact \textit{bin\_package} on $p_2+4$ symbols\\
\lno\>\>		Put (possibly compacted) \textit{bin\_package} to \textit{Compacted\_buffers\_queue}\\
\end{algorithm}
\caption{Algorithm of extra compacting bin packages prior to writing to disk.
The output of this stage are compacted packages.} 
%% \caption{Pseudocode of algorithm trying to compact bin packages even more before they are stored at HDD}
\label{code:compactor}
\end{figure}


% ***** Disk writer
\begin{figure}[h]
\begin{algorithm}{\algdef{Disk-Writer}(\textit{...})}
\pcinput{{...} --- queue with parts of FASTQ/FASTA files}\\
\pcendparam
\lno \pcwhile (\textit{bin\_id}, \textit{buffer} $\gets$ \textit{Compacted\_buffer\_queue}.pop()) \pcnot empty \pcand\\ 
\>\>\pcnot \textit{Compacted\_buffer\_queue}.finished() \pcdo\\
\lno\>	\pcif \textit{buffer} \pcnot empty \pcthen\\
\lno\>\>		Write \textit{buffer} to disk file related with \textit{bin\_id}
\end{algorithm}
\caption{Disk-writer algorithm}
\label{code:disk_writer}
\end{figure}


% ***** Bin reader
\begin{figure}[h]
\begin{algorithm}{\algdef{Bin reader}(\textit{...})}
\pcinput{{...} --- queue with parts of FASTQ/FASTA files}\\
\pcendparam
\lno \pcwhile (\textit{bin\_id} $\gets$ \textit{Bin\_ids\_queue}.pop()) \pcnot empty \pcdo\\
\lno\>	\textit{bin\_data} $\gets$ read whole file related to \textit{bin\_id}\\
\lno\>	\textit{Bins\_queue}.push(\textit{bin\_id}, \textit{bin\_data})
\end{algorithm}
\caption{Bin reader algorithm}
\label{code:bin_reader}
\end{figure}


% ***** Sorter
\begin{figure}[h]
\begin{algorithm}{\algdef{Sorter}(\textit{...})}
\pcinput{{...} --- queue with parts of FASTQ/FASTA files}\\
\pcendparam
\lno \pcwhile (\textit{bin\_id}, \textit{bin\_data} $\gets$ \textit{Bins\_queue}.pop()) \pcnot empty \pcand \pcnot \textit{Bins\_queue}.finished() \pcdo\\
\lno\>	\pcif \textit{bin\_data} \pcnot empty \pcthen\\
\lno\>\>	Uncompact $k$-mers in \textit{bin\_data}\\
\lno\>\>	Sort uncompacted $k$-mers\\
\lno\>\>	Merge identical $k$-mers removing the ones with to low or to high (out of thresholds) counter values\\
\lno\>\>	Create the buffers for save as the results\\
\lno\>\>	Put the (two) buffers ready to save to output file to \textit{Sorted\_and\_compacted\_bins\_priority\_queue}
\end{algorithm}
\caption{Sorter algorithm.}
\label{code:sorter}
\end{figure}


% ***** Completer
\begin{figure}
\begin{algorithm}{\algdef{Completer}(\textit{...})}
\pcinput{{...} --- queue with parts of FASTQ/FASTA files}\\
\pcendparam
\lno \pcwhile (\textit{bin\_id}, \textit{buffers} $\gets$ \textit{Sorted\_and\_compacted\_bins\_priority\_queue}.pop()) \pcnot empty \pcand\\
\>\> \pcnot \textit{Sorted\_and\_compacted\_bins\_priority\_queue}.finished() \pcdo\\
\lno\>	\pcif \textit{buffers} \pcnot empty \pcthen\\
\lno\>\>		Store \textit{buffers} to two output files
\end{algorithm}
\caption{Completer algorithm}
\label{code:completer}
\end{figure}










